Learning with Rejection for Abstractive Text Summarization

State-of-the-art abstractive summarization systems frequently hallucinate content that is not supported by the source document, mainly due to noise in the training dataset. Existing methods opt to drop the noisy samples or tokens from the training set entirely, reducing the effective training set size and creating an artificial propensity to copy words from the source. In this work, we propose a training objective for abstractive summarization based on rejection learning, in which the model learns whether or not to reject potentially noisy tokens. We further propose a regularized decoding objective that penalizes non-factual candidate summaries during inference by using the rejection probability learned during training. We show that our method considerably improves the factuality of generated summaries in automatic and human evaluations when compared to five baseline models and that it does so while increasing the abstractiveness of the generated summaries.

==> not_used.tex <==
% \arrayrulecolor{LightGray} 
% \begin{table*}[t!]
% \small
% % \setlength{\belowcaptionskip}{-0.5cm}
% \renewcommand{\arraystretch}{1.05}
% \centering
% \begin{tabular}{cm{13cm}}
%   \toprule
%   \Tstrut\multirow{2}{*}{Rejction} & \textbf{BART}: The University of Manchester has been awarded \tcbox[colback=LightOrange]{\pounds 3.5m} to help fund a new cancer research centre. \\
%   ~ & \textbf{Ours}: The University of Manchester has been awarded \tcbox{<reject>} \Bstrut \\
%   \hline
%   \Tstrut\multirow{2}{*}{\makecell{Factual \\ Hallucination}} & \textbf{BART}: China's Tiangong-1 space station will burn up when it re-enters the Earth's atmosphere \tcbox[colback=LightOrange]{later this week}, according to the country's space agency. \\
%   ~ & \textbf{Ours}: China's Tiangong-1 space station will burn up when it re-enters the Earth's atmosphere, Chinese officials have said. \Bstrut \\
%   \hline
%   \Tstrut\multirow{2}{*}{Rejction} & \textbf{BART}: The University of Manchester has been awarded \tcbox[colback=LightOrange]{\pounds 3.5m} to help fund a new cancer research centre. \\
%   ~ & \textbf{Ours}: The University of Manchester has been awarded \tcbox{<R>} \Bstrut \\
%   \bottomrule
% \end{tabular}
% \caption{\label{table:example} Examples of four types of hallucinations. }
% \end{table*}

% \begin{table}[t!]
% % \vspace{-1.8mm}
% % \setlength{\belowcaptionskip}{-0.3cm}
% \renewcommand{\arraystretch}{0.95}
% \begin{center}
% \begin{adjustbox}{width=.85\columnwidth, center}
% \begin{tabular}{lcc}
% \toprule
% ~ & \bf Factual Ent. & \bf Non-factual Ent. \\ 
% \midrule
% Rejection & 15.0\% & 77.6\% \\
% Same Ent. & 78.9\% & 17.2\% \\
% Different Hal. & 0.4\%  & 0.7\% \\
% Factual Ent. & 0.1\%  & 0.0\% \\
% Remove Ent. & 5.6\%  & 4.5\% \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{center}
% \caption{\label{table:rej_align} Distribution of five different types of outputs for factual and non-factual entities.}
% \end{table}

% Table \ref{tab:example} shows an example from the \textsc{XSum} test set. In this example, the beam search algorithm returns six homogeneous summaries with the only difference being the value of the funding, and these values are all non-factual. Even after increasing the beam size to 512 (we did not try larger beam sizes due to memory constraints), the results are very similar. In this case, the re-ranking based methods will not work.
